Exploring Millions of 6-State FSSP Solutions: the Formal Notion of Local CA Simulation

In this paper, we come back on the notion of local simulation allowing to transform a cellular automaton into a closely related one with different local encoding of information. This notion is used to explore solutions of the Firing Squad Synchronization Problem that are minimal both in time (2n -- 2 for n cells) and, up to current knowledge, also in states (6 states). While only one such solution was proposed by Mazoyer since 1987, 718 new solutions have been generated by Clergue, Verel and Formenti in 2018 with a cluster of machines. We show here that, starting from existing solutions, it is possible to generate millions of such solutions using local simulations using a single common personal computer.

==> tex/local-search.tex <==
\begin{algorithm}[h]
    \SetAlgoNoLine
    %\scriptsize

    \Indp
    \Indm\localsearch{$ls_\alpha, \superTransTab_\alpha, k$}\\
    \Indp
    
    $RES \gets \{ ls_\alpha \}$\\
    $LS_{current} \gets \{ ls_\alpha \}$\\
    %$y^* \gets x$\\
    \While{$\card{LS_{current}}\ > 0$}{
        $LS_{next} \gets \{\}$\\
        \For{$x \in LS_{current}$}{
            $S \gets \neighborhood(x)$\\
            $z \gets \textsf{perturbation}(x, k)$\\
            \If{$z \not\in RES$}{
                $S \gets S \union \neighborhood(z)$ \\
                \If{$\fitnessFunction(z, \superTransTab_\alpha) = 1$}{
                    $RES \gets RES \union \{z\}$
                } 
            } 
            \For{$y \in (S \setminus RES)$}{
                \If{$\fitnessFunction(y, \superTransTab_\alpha) = 1$}{
                    $LS_{next} \gets LS_{next} \cup \{y\}$\\ 
                    $RES \gets RES \cup \{y\}$
                }
            }
        }
        $LS_{current} \gets LS_{next}$
    }
    \Return $RES$
    \caption{Exploration Algorithm \mnote{Aligner les notations, e.g. $ls$ ou $g$ ou $h$ pour les local mapping ?}\mnote{Donner un meilleur nom à la fonction $f$.}}
    \label{local-search-algo}
\end{algorithm}
